Investigating a mixed action approach for {\eta} and {\eta}' mesons in Nf=2+1+1 lattice QCD

We present results for a test of a mixed action approach with Osterwalder-Seiler valence quarks on a Wilson twisted mass sea for the example {\eta}, {\eta}' mesons. Flavour singlet pseudoscalar mesons obtain significant contributions from disconnected diagrams and are, therefore, expected to be particularly sensitive to mixed regularisations. We employ different procedures for matching valence and sea quark actions and show that the results agree in the continuum limit.

==> aDepPrime.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10080.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2952,1073){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(2952,1810){\makebox(0,0)[r]{\strut{} 0}}%
      \put(2952,2547){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(2952,3284){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(2952,4021){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(2952,4758){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(2952,5495){\makebox(0,0)[r]{\strut{} 1}}%
      \put(3312,484){\makebox(0,0){\strut{} 0}}%
      \put(4453,484){\makebox(0,0){\strut{} 0.01}}%
      \put(5594,484){\makebox(0,0){\strut{} 0.02}}%
      \put(6734,484){\makebox(0,0){\strut{} 0.03}}%
      \put(7875,484){\makebox(0,0){\strut{} 0.04}}%
      \put(2182,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$r_0 \Delta M_{\eta'} $}}}%
      \put(5479,154){\makebox(0,0){\strut{}$a^2/r_0^2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6888,5322){\makebox(0,0)[r]{\strut{}$K^+$-matching}}%
      \csname LTb\endcsname%
      \put(6888,5102){\makebox(0,0)[r]{\strut{}$\eta_s$-matching}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{aDepPrime}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> aMPSDep.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10080.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3027,704){\makebox(0,0)[r]{\strut{}-0.3}}%
      \put(3027,1388){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(3027,2073){\makebox(0,0)[r]{\strut{}-0.1}}%
      \put(3027,2757){\makebox(0,0)[r]{\strut{} 0}}%
      \put(3027,3442){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(3027,4126){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(3027,4811){\makebox(0,0)[r]{\strut{} 0.3}}%
      \put(3027,5495){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(3387,484){\makebox(0,0){\strut{} 0}}%
      \put(4528,484){\makebox(0,0){\strut{} 0.01}}%
      \put(5669,484){\makebox(0,0){\strut{} 0.02}}%
      \put(6810,484){\makebox(0,0){\strut{} 0.03}}%
      \put(7951,484){\makebox(0,0){\strut{} 0.04}}%
      \put(2257,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$r_0 \Delta M_\eta $}}}%
      \put(5555,154){\makebox(0,0){\strut{}$a^2/r_0^2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4814,5043){\makebox(0,0)[r]{\strut{}$K^+$-matching}}%
      \csname LTb\endcsname%
      \put(4814,4823){\makebox(0,0)[r]{\strut{}$\eta_s$-matching}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{aMPSDep}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> angle.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10080.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2886,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(2886,1388){\makebox(0,0)[r]{\strut{} 10}}%
      \put(2886,2073){\makebox(0,0)[r]{\strut{} 20}}%
      \put(2886,2757){\makebox(0,0)[r]{\strut{} 30}}%
      \put(2886,3442){\makebox(0,0)[r]{\strut{} 40}}%
      \put(2886,4126){\makebox(0,0)[r]{\strut{} 50}}%
      \put(2886,4811){\makebox(0,0)[r]{\strut{} 60}}%
      \put(2886,5495){\makebox(0,0)[r]{\strut{} 70}}%
      \put(3202,484){\makebox(0,0){\strut{} 0}}%
      \put(4124,484){\makebox(0,0){\strut{} 0.01}}%
      \put(5045,484){\makebox(0,0){\strut{} 0.02}}%
      \put(5966,484){\makebox(0,0){\strut{} 0.03}}%
      \put(6888,484){\makebox(0,0){\strut{} 0.04}}%
      \put(7809,484){\makebox(0,0){\strut{} 0.05}}%
      \put(2248,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$\phi[\text{Deg}] $}}}%
      \put(5413,154){\makebox(0,0){\strut{}$a^2/r_0^2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6822,5322){\makebox(0,0)[r]{\strut{}$\eta_s$-matching}}%
      \csname LTb\endcsname%
      \put(6822,5102){\makebox(0,0)[r]{\strut{}$K^+$-matching}}%
      \csname LTb\endcsname%
      \put(6822,4882){\makebox(0,0)[r]{\strut{}unitary}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{angle}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> angleAMPSDep.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10080.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2961,704){\makebox(0,0)[r]{\strut{}-25}}%
      \put(2961,1183){\makebox(0,0)[r]{\strut{}-20}}%
      \put(2961,1662){\makebox(0,0)[r]{\strut{}-15}}%
      \put(2961,2141){\makebox(0,0)[r]{\strut{}-10}}%
      \put(2961,2620){\makebox(0,0)[r]{\strut{}-5}}%
      \put(2961,3100){\makebox(0,0)[r]{\strut{} 0}}%
      \put(2961,3579){\makebox(0,0)[r]{\strut{} 5}}%
      \put(2961,4058){\makebox(0,0)[r]{\strut{} 10}}%
      \put(2961,4537){\makebox(0,0)[r]{\strut{} 15}}%
      \put(2961,5016){\makebox(0,0)[r]{\strut{} 20}}%
      \put(2961,5495){\makebox(0,0)[r]{\strut{} 25}}%
      \put(3321,484){\makebox(0,0){\strut{} 0}}%
      \put(4462,484){\makebox(0,0){\strut{} 0.01}}%
      \put(5603,484){\makebox(0,0){\strut{} 0.02}}%
      \put(6744,484){\makebox(0,0){\strut{} 0.03}}%
      \put(7885,484){\makebox(0,0){\strut{} 0.04}}%
      \put(2323,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$\Delta \phi\text{[Deg]}$}}}%
      \put(5489,154){\makebox(0,0){\strut{}$a^2/r_0^2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6898,5322){\makebox(0,0)[r]{\strut{}$K^+$-matching}}%
      \csname LTb\endcsname%
      \put(6898,5102){\makebox(0,0)[r]{\strut{}$\eta_s$-matching}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{angleAMPSDep}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> mPSDep.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10080.00,8640.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,2622){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,4540){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1078,6457){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1078,8375){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1210,484){\makebox(0,0){\strut{} 0}}%
      \put(2430,484){\makebox(0,0){\strut{} 0.2}}%
      \put(3650,484){\makebox(0,0){\strut{} 0.4}}%
      \put(4870,484){\makebox(0,0){\strut{} 0.6}}%
      \put(6089,484){\makebox(0,0){\strut{} 0.8}}%
      \put(7309,484){\makebox(0,0){\strut{} 1}}%
      \put(8529,484){\makebox(0,0){\strut{} 1.2}}%
      \put(9749,484){\makebox(0,0){\strut{} 1.4}}%
      \put(308,4539){\rotatebox{-270}{\makebox(0,0){\strut{}$r_0 M_{\eta,\eta'} $}}}%
      \put(5479,154){\makebox(0,0){\strut{}($r_0 M_{PS})^2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5698,8202){\makebox(0,0)[r]{\strut{}A ensemble}}%
      \csname LTb\endcsname%
      \put(5698,7982){\makebox(0,0)[r]{\strut{}A ensemble, unitaer}}%
      \csname LTb\endcsname%
      \put(5698,7762){\makebox(0,0)[r]{\strut{}B ensemble}}%
      \csname LTb\endcsname%
      \put(5698,7542){\makebox(0,0)[r]{\strut{}B ensemble, unitaer}}%
      \csname LTb\endcsname%
      \put(5698,7322){\makebox(0,0)[r]{\strut{}D ensemble}}%
      \csname LTb\endcsname%
      \put(5698,7102){\makebox(0,0)[r]{\strut{}D ensemble, unitaer}}%
      \csname LTb\endcsname%
      \put(5698,6882){\makebox(0,0)[r]{\strut{}$b=0.41\pm 0.12 ~ a=2.69 \pm0.14$}}%
      \csname LTb\endcsname%
      \put(5698,6662){\makebox(0,0)[r]{\strut{}$b=0.42 \pm 0.6 ~ a=1.98\pm 0.07$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mPSDep}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> mass.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10080.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2952,1073){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(2952,1810){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(2952,2547){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(2952,3284){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(2952,4021){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(2952,4758){\makebox(0,0)[r]{\strut{} 1.7}}%
      \put(2952,5495){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(3268,484){\makebox(0,0){\strut{} 0}}%
      \put(4190,484){\makebox(0,0){\strut{} 0.01}}%
      \put(5111,484){\makebox(0,0){\strut{} 0.02}}%
      \put(6032,484){\makebox(0,0){\strut{} 0.03}}%
      \put(6954,484){\makebox(0,0){\strut{} 0.04}}%
      \put(7875,484){\makebox(0,0){\strut{} 0.05}}%
      \put(2182,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$r_0 M_\eta $}}}%
      \put(5479,154){\makebox(0,0){\strut{}$a^2/r_0^2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4717,5201){\makebox(0,0)[r]{\strut{}$\eta_s$-matching}}%
      \csname LTb\endcsname%
      \put(4717,4981){\makebox(0,0)[r]{\strut{}$K^+$-matching}}%
      \csname LTb\endcsname%
      \put(4717,4761){\makebox(0,0)[r]{\strut{}unitary}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mass}}%
    \gplfronttext
  \end{picture}%
\endgroup

